On Decoding High-Order Interleaved Sum-Rank-Metric Codes

We consider decoding of vertically homogeneous interleaved sum-rank-metric codes with high interleaving order $s$, that are constructed by stacking $s$ codewords of a single constituent code. We propose a Metzner--Kapturowski-like decoding algorithm that can correct errors of sum-rank weight $t <= d-2$, where $d$ is the minimum distance of the code, if the interleaving order $s > t$ and the error matrix fulfills a certain rank condition. The proposed decoding algorithm generalizes the Metzner--Kapturowski(-like) decoders in the Hamming metric and the rank metric and has a computational complexity of $\tilde{O}(\max(n^3, n^2 s))$ operations in $\mathbb{F}_{q^m}$, where $n$ is the length of the code. The scheme performs linear-algebraic operations only and thus works for any interleaved linear sum-rank-metric code. We show how the decoder can be used to decode high-order interleaved codes in the skew metric. Apart from error control, the proposed decoder allows to determine the security level of code-based cryptosystems based on interleaved sum-rank metric codes.

==> sections/generalizations.tex <==
%----------------------------------------------------------------------------
% Generalizations
%----------------------------------------------------------------------------
\section{Generalizations of the Decoding Schemes} \label{sec:generalizations}

\begin{itemize}
    \item Comment on correcting more than $d-2$ errors (cf.~\cite[Section~IV-C]{puchinger2019decoding}) \hb{In~\cite{oh1994performance} Oh and Metzner considered this case for the Hamming metric (paper not cited in~\cite{puchinger2019decoding}).} \\
        $\Rightarrow$ should be straight forward \todo{HB}
        
        \item Comment on heterogeneous interleaved codes (cf.~\cite[Section~IV-D]{puchinger2019decoding}) \\
        $\Rightarrow$ should be straight forward
        

        \item In~\cite{haslach2000efficient}, Haslach and Han Vinck (which proposed the Metzner--Kapturowski decoder~\cite{metzner1990general} independently in~\cite{haslach1999decoding}) extended the Metzner--Kapturowski decoder in the Hamming metric to $\Fqm$-linear dependent error matrices, i.e. error matrices $\E\in\Fqm^{\intOrder \times n}$ with $\rk_{q^m}(\E) < t$. The (guaranteed) decoding capability is then given by (see~\cite[Equation~1]{haslach2000efficient})
        \begin{equation}
            t \leq d -2 - (t-\rk_{q^m}(\E)).
        \end{equation}
        Can we get a similar result for our decoder?
        This result is still open for the rank-metric (see~\cite[Section~V-B]{puchinger2019decoding}).
        See also~\cite[Sectio~II.A]{roth2014coding} and~\cite[Section~IV.B]{holzbaur2021decoding} for more insights on the error-correction capability for $\Fqm$-linearly dependent errors~\cite{haslach2000efficient}.

        \begin{itemize}
            \item Note, that if $\mu \defeq \rkqm(\E)<t$, then Lemma~\ref{lem:row_space_H_sub} still holds, i.e. we have that 
            \begin{equation}
                \RowspaceFqm{\Hsub}=\rker(\E)_{q^m} \cap \RowspaceFqm{\H}.
            \end{equation}
            However, we get $n-k-\mu$ all-zero rows in $\REF(\S)$ and therefore we have that $\Hsub\in\Fqm^{(n-k-\mu) \times n}$.

            \item Even if $\mu <t$ we might have that $\rkqm(\E^{(i)})=t_i$ for some $i\in\{1,\dots,\shots\}$. 
            Let $\set{J} \defeq \{i\in\{1,\dots,\shots\}:\rkqm(\E^{(i)})=t_i\}$ the set of indices $i$ for which $\rkqm(\E^{(i)})=t_i$.
            Then by Lemma~\ref{lem:Fqm_kernel_Ei_Bi} we have that
            \begin{equation}
                 \rker(\E^{(i)})_{q^m}=\rker(\B^{(i)})_{q^m}, \quad\forall i \in \set{J}
            \end{equation} 
            if $\intOrder \geq \max_i\{t_i\}$, which holds if the high-order condition $\intOrder \geq t$ is satisfied.
            Therefore, we can recover the row space of $\B^{(i)}$ from the right kernel of $\ext(\Hsub^{(i)})$ for all blocks indexed by $\set{J}$ (this is due to the fact that in the proof of Theorem~\ref{thm:sum_rank_support_recovery} we argue on a block-diagonal matrix), which we may in turn use for erasure decoding. 
            \hb{This only works in the sum-rank metric for $\shots > 1$ blocks!}
        \end{itemize}

        \item Show how we can use the decoder for the skew metric \\
        $\Rightarrow$ here we might have to fix a basis and an evaluation parameter per block and use interpolation polynomials in order to use the isometry between the sum-rank and the skew metric~\cite[Theorems~2~\&~3]{martinez2018skew} for vectors and non-evaluation codes. \todo{HB} \hb{Maybe put into separate section}
\end{itemize}
